SandboxAQ's submission to MRL 2024 Shared Task on Multi-lingual Multi-task Information Retrieval

This paper explores the problems of Question Answering (QA) and Named Entity Recognition (NER) in five diverse languages. We tested five Large Language Models with various prompting methods, including zero-shot, chain-of-thought reasoning, and translation techniques. Our results show that while some models consistently outperform others, their effectiveness varies significantly across tasks and languages. We saw that advanced prompting techniques generally improved QA performance but had mixed results for NER; and we observed that language difficulty patterns differed between tasks. Our findings highlight the need for task-specific approaches in multilingual NLP and suggest that current models may develop different linguistic competencies for different tasks.

==> plot_qa_bars.tex <==
\begin{figure*}[t]

\newpage
\subsection{Best QA and NER performance figures}
\label{sec:appendix_figures}
\vspace{2mm}
\hspace*{-1cm}\centering
\begin{tikzpicture}[scale=1]
\begin{axis}[
    width=1.1\textwidth,
    height=0.5\textheight,
    ylabel={Accuracy (\%)},
    xlabel={Language},
    ymin=0, ymax=100,
    symbolic x coords={ALS,YO,AZ,IG,TR},
    xtick=data,
    enlarge x limits=0.15,
    clip=false,
    legend style={
        at={(0.5,1.25)},
        anchor=south,
        legend columns=3,
        font=\footnotesize
    },
    ylabel near ticks,
    ybar=1.5pt,
    bar width=3pt,
    title={QA Performance: gpt-4o vs gpt-4-turbo vs claude-3.5-sonnet},
    title style={
        at={(0.5,1)},
        anchor=south,
        font=\large
    },
]

% gpt-4o
\addplot[fill=purple!100] coordinates {
    (ALS,94.10) (YO,94.10) (AZ,98.00) (IG,98.20) (TR,96.92)
};
\addplot[fill=purple!80] coordinates {
    (ALS,92.50) (YO,90.00) (AZ,97.50) (IG,97.00) (TR,95.38)
};
\addplot[fill=purple!60] coordinates {
    (ALS,91.50) (YO,91.50) (AZ,92.00) (IG,91.50) (TR,91.79)
};
\addplot[fill=purple!40] coordinates {
    (ALS,89.50) (YO,90.00) (AZ,89.52) (IG,90.00) (TR,89.74)
};
\addplot[fill=purple!20] coordinates {
    (ALS,91.60) (YO,88.90) (AZ,94.80) (IG,96.70) (TR,96.82)
};
\addplot[fill=purple!10] coordinates {
    (ALS,97.04) (YO,95.50) (AZ,97.00) (IG,95.02) (TR,96.92)
};

% gpt-4-turbo
\addplot[fill=orange!100] coordinates {
    (ALS,88.20) (YO,90.10) (AZ,96.63) (IG,95.50) (TR,95.18)
};
\addplot[fill=orange!80] coordinates {
    (ALS,97.00) (YO,93.00) (AZ,99.00) (IG,96.50) (TR,96.23)
};
\addplot[fill=orange!60] coordinates {
    (ALS,96.50) (YO,97.00) (AZ,98.00) (IG,98.50) (TR,97.59)
};
\addplot[fill=orange!40] coordinates {
    (ALS,97.50) (YO,99.00) (AZ,98.50) (IG,96.50) (TR,96.92)
};
\addplot[fill=orange!20] coordinates {
    (ALS,95.50) (YO,95.00) (AZ,97.50) (IG,96.50) (TR,97.44)
};
\addplot[fill=orange!10] coordinates {
    (ALS,97.50) (YO,97.84) (AZ,98.00) (IG,98.01) (TR,97.86)
};

% claude-3.5-sonnet
\addplot[fill=teal!100] coordinates {
    (ALS,92.50) (YO,94.50) (AZ,99.50) (IG,93.00) (TR,96.92)
};
\addplot[fill=teal!80] coordinates {
    (ALS,95.00) (YO,96.00) (AZ,94.00) (IG,94.50) (TR,94.87)
};
\addplot[fill=teal!60] coordinates {
    (ALS,93.00) (YO,91.50) (AZ,92.00) (IG,91.00) (TR,92.82)
};
\addplot[fill=teal!40] coordinates {
    (ALS,92.00) (YO,92.00) (AZ,94.50) (IG,95.00) (TR,96.41)
};
\addplot[fill=teal!20] coordinates {
    (ALS,92.00) (YO,90.00) (AZ,98.00) (IG,94.00) (TR,97.44)
};
\addplot[fill=teal!10] coordinates {
    (ALS,93.00) (YO,98.50) (AZ,99.00) (IG,94.50) (TR,96.92)
};

\legend{
  gpt-4o,
  gpt-4o + T,
  gpt-4o DSPy CoT,
  gpt-4o DSPy CoT + T,
  gpt-4o DSPy ReAct,
  gpt-4o DSPy ReAct + T,
  gpt-4-turbo,
  gpt-4-turbo + T,
  gpt-4-turbo DSPy CoT,
  gpt-4-turbo DSPy CoT + T,
  gpt-4-turbo DSPy ReAct,
  gpt-4-turbo DSPy ReAct + T,
  claude-3.5-sonnet,
  claude-3.5-sonnet + T,
  claude-3.5-sonnet DSPy CoT,
  claude-3.5-sonnet DSPy CoT + T,
  claude-3.5-sonnet DSPy ReAct,
  claude-3.5-sonnet DSPy ReAct + T
}

% Adjusted labels for the highest values
%\node[anchor=west, rotate=90, font=\footnotesize] at (axis cs:ALS,97.50) {97.50\%}; % gpt-4-turbo DSPy CoT + T
%\node[anchor=west, rotate=90, font=\footnotesize] at (axis cs:YO,99.00) {99.00\%}; % gpt-4-turbo DSPy CoT + T
%\node[anchor=west, rotate=90, font=\footnotesize] at (axis cs:AZ,99.50) {99.50\%}; % claude-3.5-sonnet
%\node[anchor=west, rotate=90, font=\footnotesize] at (axis cs:IG,98.50) {98.50\%}; % gpt-4-turbo DSPy CoT
%\node[anchor=west, rotate=90, font=\footnotesize] at (axis cs:TR,97.86) {97.86\%}; % gpt-4-turbo DSPy ReAct + T

\end{axis}
\end{tikzpicture}
\caption{Comparison of QA performance (Accuracy \%) between the three best performing models, gpt-4o, gpt-4-turbo, and claude-3.5-sonnet, across all languages and methods. {+} T indicates the {+} Translation experiment.}
\label{fig:comprehensive-qa-performance}
\end{figure*}
